An Alternative Approach to Functional Linear Partial Quantile Regression

Functional data such as curves and surfaces have become more and more common with modern technological advancements. The use of functional predictors remains challenging due to its inherent infinite-dimensionality. The common practice is to project functional data into a finite dimensional space. The popular partial least square (PLS) method has been well studied for the functional linear model [1]. As an alternative, quantile regression provides a robust and more comprehensive picture of the conditional distribution of a response when it is non-normal, heavy-tailed, or contaminated by outliers. While partial quantile regression (PQR) was proposed in [2], no theoretical guarantees were provided due to the iterative nature of the algorithm and the non-smoothness of quantile loss function. To address these issues, we propose an alternative PQR (APQR) formulation with guaranteed convergence. This novel formulation motivates new theories and allows us to establish asymptotic properties. Numerical studies on a benchmark dataset show the superiority of our new approach. We also apply our novel method to a functional magnetic resonance imaging (fMRI) data to predict attention deficit hyperactivity disorder (ADHD) and a diffusion tensor imaging (DTI) dataset to predict Alzheimer's disease (AD).

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


